Differentiable Weightless Neural Networks

We introduce the Differentiable Weightless Neural Network (DWN), a model based on interconnected lookup tables. Training of DWNs is enabled by a novel Extended Finite Difference technique for approximate differentiation of binary values. We propose Learnable Mapping, Learnable Reduction, and Spectral Regularization to further improve the accuracy and efficiency of these models. We evaluate DWNs in three edge computing contexts: (1) an FPGA-based hardware accelerator, where they demonstrate superior latency, throughput, energy efficiency, and model area compared to state-of-the-art solutions, (2) a low-power microcontroller, where they achieve preferable accuracy to XGBoost while subject to stringent memory constraints, and (3) ultra-low-cost chips, where they consistently outperform small models in both accuracy and projected hardware area. DWNs also compare favorably against leading approaches for tabular datasets, with higher average rank. Overall, our work positions DWNs as a pioneering solution for edge-compatible high-throughput neural networks.

==> 00_abstract.tex <==
% ICML asks for around 6 phrases. Most ICML papers have < 200 words, with avg of 120-160.
\begin{abstract}
% Weightless neural networks use binary weights in look up tables (LUTs) and are not traditionally differentiable. In this paper, we present weightless neural networks that use multilayer LUTs and employ techniques of extended finite differences, learnable mapping, learnable reduction, spectral normalization and polynominal relaxation to allow reliable training to improved accuracies and reduced hardware requirements.  In comparison to DiffLogicNet, the presented models achieve 7\% higher accuracy for Keyword Spotting and 3\% higher accuracy for ToyAdmos intrusion detection datasets. For tabular data, our models are competitive in comparison to state-of-the-art tabular models such as XGBoost and other techniques in AutoGluon, Google TabNet, showing that our model efficiency does not come at the cost of accuracy.

Our research introduces the Differentiable Weightless Neural Network (DWNN), a type of lookup table (LUT)-based neural networks
%advancing beyond traditional single-layer Weightless Neural Networks (WNNs) 
by introducing the Extended Finite Differences technique for approximate differentiation of binary values. We further enhance DWNNs with novel techniques such as Learnable Mapping, Learnable Reduction, and Spectral Normalization, significantly improving training, accuracy, and hardware efficiency. DWNNs outperform Binary Neural Networks (BNNs) in the MLPerfTiny KWS benchmark, achieving an 8.9x reduction in LUT usage, a 15.7x increase in throughput, and a 135x decrease in energy costs. In tabular data, the DWNN surpasses state-of-the-art tabular models such as XGBoost and TabNets, achieving an improved rank of 2.5 compared to average ranks of 3.4 and 3.6 respectively. For ultra-low-cost chip implementations, DWNNs demonstrate up to a 42.8x reduction in NAND2 circuit size compared to leading Tiny Classifiers~\cite{tinyclassifier}. These position the DWNN as a pioneering solution for edge-compatible high-throughput neural networks. \rt{Add  arduino results}. \rt{Add  arduino results

\begin{comment}
We introduce the Differentiable Weightless Neural Network (DWNN), a lookup table (LUT)-based neural model.
Training of DWNNs is enabled by the novel Extended Finite Difference technique for approximate differentiation of binary values.
We further enhance DWNNs with original techniques such as Learnable Mapping, Learnable Reduction, and Spectral Normalization, significantly improving model accuracy and efficiency.


\end{comment}


\end{abstract}

==> 01_introduction.tex <==
\section{Introduction}

The field of deep learning has witnessed remarkable advancements in recent years, leading to significant innovations across various domains \cite{imagenet_cnn, cnn_deeper, acoustic_hinton, translation1, translation2}.  However, this rapid progression has been accompanied by escalating computational demands, posing a substantial challenge in deploying efficient models for inference, especially in resource-constrained environments. The need for high computational resources limits the applicability of advanced deep learning models in settings where energy and processing power are at a premium, such as edge computing and mobile devices. (\textcolor{green}{Figure 1 is in the wrong place. It should be close to where we refer to Figure 1 for the very first time)}

Numerous approaches have been proposed to mitigate these computational costs, including techniques like pruning \cite{prune1, prune2, prune3}, quantization \cite{quantization1, quantization2, quantization3}, and the development of sparse neural networks \cite{quantization1, quantization2, quantization3}. While these strategies have been effective in reducing the overall amount of computation required, they do not fundamentally address the high intrinsic costs associated with multiplication operations in neural networks. This limitation remains a significant hurdle in the quest for highly efficient deep learning models.

\begin{figure}[t]
\centerline{\includegraphics[width=0.95\columnwidth]{figures/iris_alt.pdf}}
\caption{A very simple DWNN for the Iris~\cite{misc_iris_53} dataset, constructed using three-input RAMs. Computation is performed using direct table lookups during both training and inference.}
\label{fig:iris}
\end{figure}

In response to this challenge, there's been an increasing focus on developing models that do not require multiplication. A prime example is Binary Neural Networks (BNNs) \cite{bnn}, which limit weights to binary values and utilize XOR operations instead of multiplication. Other innovative models include AdderNets \cite{addernet}, which employ addition operations exclusively; DeepShift \cite{deepshift}, replacing multiplication with bit shifting; and the more recent DiffLogicNets \cite{difflogicnet}, which are trained to learn logic gate networks. These approaches have been effectively implemented across a range of applications, underscoring the practicality and potential of multiplication-free architectures \cite{bnnapp1, bnnapp3, bnnapp4, bnnapp5}.

Within this context, Weightless Neural Networks (WNNs) stand out as a distinct category. Diverging from the norm, WNNs forgo traditional weighted connections, opting instead for lookup tables (LUTs) with binary values to drive neural activity \cite{wisard}. This unique approach not only allows for high computational efficiency \cite{uleen} but also empowers WNNs to adeptly learn complex functions, highlighted by their significant VC-dimension \cite{vc_wi}. %As a result, WNNs has found successful applications across various domains \cite{wnnapp1, wnnapp2, wnnapp3, wnnapp4}.

However, a notable limitation of WNNs has been their restriction to single-layer architectures. This constraint is primarily due to the discrete structure of LUTs, which has historically prevented the development of deep, multi-layer WNNs. % Consequently, WNNs have generally been confined to simpler computational tasks.

Despite this limitation, recent advancements have illuminated the potential of WNNs for achieving high efficiency in neural computation. The ULEEN model \cite{uleen} exemplifies this, showcasing a WNN's capabilities on an FPGA platform. Remarkably, ULEEN has outperformed BNNs in accuracy, energy efficiency, latency, memory consumption and circuit area. This is particularly noteworthy considering that ULEEN operates with a single-layer structure, in contrast to the deep architecture of BNNs. This success not only underscores the inherent efficiency of WNNs but also implies the immense potential they could unlock if developed beyond their current single-layer constraints.

% Contributions and results in sentences style
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Recognizing the critical need for innovation in this area, our work introduces two groundbreaking methods: \textbf{Extended Finite Differences (EFD)} and \textbf{Polynomial Relaxation (PR)}. These techniques enable backpropagation through LUTs, thereby paving the way for the development of deep WNN architectures. This advancement has the potential to revolutionize the field of deep learning by enabling the development of more complex WNN models. Furthermore, three more novels techniques that improves training, accuracy, and hardware efficiency. These are:  \textbf{Learnable Mapping}, a innovative layer allows DWNNs to learn connections between LUTs during training, moving beyond fixed or random setups in WNNs and enhancing adaptability and efficiency without additional overhead during inference; \textbf{Leranable Reduction}, tailored for very tiny models, this approach facilitates the learning of class discrimination during training, leading to smaller and more efficient models; and \textbf{Spectral Regularization}, a specialized normalization technique tailored for LUTs in WNNs.

% Our results demonstrates the DWNN's versatility and efficacy in various scenarios: (1) In FPGA deployment, the DWNN outperforms Binary Neural Networks (BNNs), ULEEN, and DiffLogicNets, exhibiting substantial improvements in LUT usage, throughput, and energy efficiency across all tested datasets, and showing effective hardware-software co-design by aligning LUT sizes with FPGA's native CLB size. (2) In constrained edge devices, such as the Arduino Nano, our compact model architecture achieves significantly superior accuracy compared to models like XGBoost. (3) For ultra-low-cost chip implementations, the DWNN impressively reduces circuit area compared to leading Tiny Classifier models, again leveraging hardware-software co-design. (4) In the analysis of tabular data, the DWNN surpasses state-of-the-art models such as XGBoost and TabNets, achieving the highest average rank among all evaluated models.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Contributions and results in bullet points style
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Recognizing the critical need for innovation in this area, our work introduces the \textbf{Differentiable Weightless Neural Network (DWNN)}. This is achieved with a suite of innovative techniques:
\vspace{-3mm}
\begin{itemize}[leftmargin=*]
\setlength\itemsep{-3pt}
\item \textbf{Extended Finite Difference:}
 This technique enables backpropagation through LUTs by approximate differentiation, allowing the development of Multi-layer WNN architectures.
%\vspace{-3mm}
\item \textbf{Learnable Mapping:} This innovative layer allows DWNNs to learn connections between LUTs during training, moving beyond fixed or random setups in WNNs and enhancing adaptability and efficiency without additional overhead during inference.
%\vspace{-2.2mm}
\item \textbf{Learnable Reduction:} Tailored for very tiny models, this approach facilitates the learning of class discrimination during training, leading to smaller and more efficient models.
%\vspace{-2mm}
\item \textbf{Spectral Normalization:} A normalization technique specifically developed for LUTs in WNNs {\color{blue} to avoid overfitting}.
\end{itemize}
\vspace{-2mm}
Our results demonstrates the DWNN's versatility and efficacy in various scenarios: 
\vspace{-3mm}
\begin{enumerate}[leftmargin=*]
\setlength\itemsep{-3pt}
\item \textbf{FPGA deployment}: DWNN outperforms \zjs{fully-connected BNNs and prior WNNs in latency, throughput, energy efficiency, and model area across all tested datasets by aligning model LUTs with the FPGA's native LUT size, achieving a geometric average 2522$\times$ improvement in energy-delay product versus Xilinx FINN and a 63$\times$ improvement versus ULEEN.}
%BNNs, ULEEN, and DiffLogicNets, exhibiting substantial improvements in LUT usage, throughput, and energy efficiency across all tested datasets, and showing effective hardware-software co-design by aligning LUT sizes with FPGA's native CLB size. 
%\vspace{-3mm}
\item \textbf{Constrained edge devices}: On a low-end microcontroller (Elegoo Nano), our compact model architecture achieves superior accuracy compared to XGBoost, with an average of 5.4\% improvement, albeit at the cost of significantly increased execution time.
%up to 18.6\% improvement,
%\vspace{-3mm}
\item \textbf{Ultra-low-cost chips:} The DWNN reduces circuit area by up to 42.8x compared to leading Tiny Classifier models, and up to 398x compared to DiffLogicNets.
%\vspace{-3mm}
\item \textbf{Tabular data}: DWNN surpasses state-of-the-art models such as XGBoost and TabNets, achieving an average rank of 2.5 compared to 3.4 and 3.6 respectively.
\end{enumerate}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace{-2mm}
% The culmination of these developments could mark a new epoch in neural network design, heralding a future where advanced DWNN models drive innovation across a multitude of applications. (\textcolor{green}{This is a strong statement. Is this true only for edge devices or true for all neural networks?)}

==> 01_introduction2.tex <==
\section{Introduction}
In the relentless advancements of deep learning, optimizing computational efficiency, especially at inference, remains a critical challenge. Efforts to mitigate computational demands have led to innovations in model pruning \cite{prune1, prune2, prune3}, quantization \cite{quantization1, quantization2, quantization3}, and sparse neural networks \cite{quantization1, quantization2, quantization3}. However, these approaches do not directly address the core issue associated with the multiplication operations inherent in neural networks. Consequently, research has shifted towards developing multiplication-free architectures such as Binary Neural Networks (BNNs) \cite{bnn}, AddNets \cite{addernet}, and DeepShift \cite{deepshift}, which demonstrate impressive computational efficiencies \cite{bnnapp1, bnnapp3, bnnapp4}.

\begin{figure}[t]
\centerline{\includegraphics[width=0.95\columnwidth]{figures/iris_alt.pdf}}
\caption{A very simple DWNN for the Iris~\cite{misc_iris_53} dataset, constructed using three-input RAMs. Computation is performed using direct table lookups during both training and inference.}
\label{fig:iris}
\vspace{-5mm}
\end{figure}


Among these developments, Differentiable Logic Gate Networks (DiffLogicNets) \cite{difflogicnet} have emerged as a novel paradigm, proposing a gradient descent-based method for training logic gate networks. This approach defines a new state-of-the-art for compact models, surpassing Binary Neural Networks (BNNs). DiffLogicNets learns to configure logic gate networks using two input binary logic nodes as neurons, arranging them as a feedforward neural network. Each binary node is learned with a technique encompassing a continuous relaxation of all possible two-input binary logic operators, enabling gradient descent training and back-propagation through the network layers.

Interestingly, this model represents both a rediscovery and an enhancement of Weightless Neural Networks (WNNs) \cite{wisard}, which utilize lookup tables (LUTs) with binary values as neurons—eschewing multiply and accumulate operations (MAC). The number of inputs to the LUT, \(n\), serves as a hyperparameter. The hypothesis space of DiffLogicNets' two-input binary nodes is exactly the same as a WNN with two-input LUTs (\(n=2\)). Nevetheless, as WNNs have historically been constrained to single-layer architectures due to the discrete nature of LUTs, the continuous relaxation of binary logic introduced by DiffLogicNets marks a significant improvement, enabling backpropagation through WNN's LUTs.

However, the DiffLogicNets method is only computationally feasible for very small LUTs, as their training strategy requires weights and computations on a super-exponential complexity of \(\mathcal{O}(2^{2^n})\). For example, for LUT6 (\(n=6\)), this method necessitates an astounding 18,446,744,073,709,551,616 weights and computations per LUT! The inability to train WNNs with larger LUTs is detrimental for two main reasons: (1) the VC dimension of WNNs is exponentially proportional to the number of inputs to the LUTs, making a WNN with fewer but larger LUTs a more capable learner than one with many small LUTs \cite{vc_wi}; (2) enabling the training of LUTs of varying sizes facilitates hardware-software co-design, leading to more efficient models. For instance, a LUT6-based WNN could be significantly more efficient on modern FPGAs, which employ LUT6s in their configurable logic blocks (CLBs), aligning WNN implementation more closely with FPGA architecture.

Furthermore, both WNN and DiffLogicNets currently have three other vital limitations. Firstly, they rely on pseudo-random connections between LUTs, which leaves the optimal arrangement of the neural network to chance. Secondly, the reliance on popcount for determining the activation values of each class can lead to the requirement of large circuit sizes, with the popcount circuit size being as large as the network itself. Lastly, the binary nature of LUTs means that traditional DNN regularization techniques are ineffective, thus there is a pressing need for the development of specialized regularization techniques.

Recognizing the critical need for innovation in this area, our work introduces the \textbf{Differentiable Weightless Neural Network (DWNN)}, tackling all of these limitations. This is achieved with a suite of innovative techniques:

% In recognition of the critical need for innovation in this domain, our work introduces the \textbf{Differentiable Weightless Neural Network (DWNN)}. We propose a new technique that allows WNN LUTs to undergo backpropagation with a exponential improvement in complexity, \(\mathcal{O}(2^n)\), enabling the training and deployment of larger LUT sizes. Furthermore, we introduce three additional novel techniques that further enhance the capabilities of WNNs. Here is a summary of our contributions:
\vspace{-3mm}
\begin{itemize}[leftmargin=*]
\setlength\itemsep{-3pt}
\item \textbf{Extended Finite Difference:}
 This technique enables efficient backpropagation through LUTs by approximate differentiation, allowing the development of Multi-layer WNN architectures with bigger LUTs.
%\vspace{-3mm}
\item \textbf{Learnable Mapping:} This innovative layer allows DWNNs to learn cthe onnections between LUTs during training, moving beyond fixed or random setups in WNNs and DiffLogicNets, enhancing adaptability and efficiency without additional overhead during inference.
%\vspace{-2.2mm}
\item \textbf{Learnable Reduction:} Tailored for tiny models, this approach replaces popcount with decreasing pyramidal LUT layers, leading to smaller circuit sizes.
%\vspace{-2mm}
\item \textbf{Spectral Normalization:} A normalization technique specifically developed for LUTs in WNNs {\color{blue} to avoid overfitting}.
\end{itemize}
\vspace{-2mm}
Our results demonstrates the DWNN's versatility and efficacy in various scenarios: 
\vspace{-3mm}
\begin{enumerate}[leftmargin=*]
\setlength\itemsep{-3pt}
\item \textbf{FPGA deployment}: DWNN outperforms DiffLogicNets, fully-connected BNNs and prior WNNs in latency, throughput, energy efficiency, and model area across all tested datasets by aligning model LUTs with the FPGA's native LUT size, achieving a geometric average 2522$\times$ improvement in energy-delay product versus the FINN BNN platform and a 63$\times$ improvement versus ULEEN, the current state-of-the-art for efficient WNNs.
%BNNs, ULEEN, and DiffLogicNets, exhibiting substantial improvements in LUT usage, throughput, and energy efficiency across all tested datasets, and showing effective hardware-software co-design by aligning LUT sizes with FPGA's native CLB size. 
%\vspace{-3mm}
\item \textbf{Constrained edge devices}: On a low-end microcontroller (Elegoo Nano), our compact model architecture achieves superior accuracy compared to XGBoost, with an average of 5.4\% improvement, albeit at the cost of significantly increased execution time.
%up to 18.6\% improvement,
%\vspace{-3mm}
\item \textbf{Ultra-low-cost chips:} The DWNN reduces circuit area by up to 42.8x compared to leading Tiny Classifier models, and up to 398x compared to DiffLogicNets.
%\vspace{-3mm}
\item \textbf{Tabular data}: DWNN surpasses state-of-the-art models such as XGBoost and TabNets, achieving an average rank of 2.5 compared to 3.4 and 3.6 respectively.
\end{enumerate}
